Joint Optimization of Signal Design and Resource Allocation in Wireless D2D Edge Computing

In this paper, we study the distributed computational capabilities of device-to-device (D2D) networks. A key characteristic of D2D networks is that their topologies are reconfigurable to cope with network demands. For distributed computing, resource management is challenging due to limited network and communication resources, leading to inter-channel interference. To overcome this, recent research has addressed the problems of wireless scheduling, subchannel allocation, power allocation, and multiple-input multiple-output (MIMO) signal design, but has not considered them jointly. In this paper, unlike previous mobile edge computing (MEC) approaches, we propose a joint optimization of wireless MIMO signal design and network resource allocation to maximize energy efficiency. Given that the resulting problem is a non-convex mixed integer program (MIP) which is prohibitive to solve at scale, we decompose its solution into two parts: (i) a resource allocation subproblem, which optimizes the link selection and subchannel allocations, and (ii) MIMO signal design subproblem, which optimizes the transmit beamformer, transmit power, and receive combiner. Simulation results using wireless edge topologies show that our method yields substantial improvements in energy efficiency compared with cases of no offloading and partially optimized methods and that the efficiency scales well with the size of the network.

==> Infocom.bbl.tex <==
% Generated by IEEEtran.bst, version: 1.14 (2015/08/26)
\begin{thebibliography}{10}
\providecommand{\url}[1]{#1}
\csname url@samestyle\endcsname
\providecommand{\newblock}{\relax}
\providecommand{\bibinfo}[2]{#2}
\providecommand{\BIBentrySTDinterwordspacing}{\spaceskip=0pt\relax}
\providecommand{\BIBentryALTinterwordstretchfactor}{4}
\providecommand{\BIBentryALTinterwordspacing}{\spaceskip=\fontdimen2\font plus
\BIBentryALTinterwordstretchfactor\fontdimen3\font minus
  \fontdimen4\font\relax}
\providecommand{\BIBforeignlanguage}[2]{{%
\expandafter\ifx\csname l@#1\endcsname\relax
\typeout{** WARNING: IEEEtran.bst: No hyphenation pattern has been}%
\typeout{** loaded for the language `#1'. Using the pattern for}%
\typeout{** the default language instead.}%
\else
\language=\csname l@#1\endcsname
\fi
#2}}
\providecommand{\BIBdecl}{\relax}
\BIBdecl

\bibitem{chiang2016fog}
M.~Chiang and T.~Zhang, ``{Fog and IoT: An overview of research
  opportunities},'' \emph{IEEE Internet of Things Journal}, vol.~3, no.~6, pp.
  854--864, 2016.

\bibitem{yao2019edgeflow}
C.~Yao, X.~Wang, Z.~Zheng, G.~Sun, and L.~Song, ``Edgeflow: Open-source
  multi-layer data flow processing in edge computing for {5G} and beyond,''
  \emph{IEEE Network}, vol.~33, no.~2, pp. 166--173, 2019.

\bibitem{yang2018communication}
X.~Yang, Z.~Chen, K.~Li, Y.~Sun, N.~Liu, W.~Xie, and Y.~Zhao,
  ``Communication-constrained mobile edge computing systems for wireless
  virtual reality: Scheduling and tradeoff,'' \emph{IEEE Access}, vol.~6, pp.
  16\,665--16\,677, 2018.

\bibitem{8319323}
R.~{Schmoll}, S.~{Pandi}, P.~J. {Braun}, and F.~H.~P. {Fitzek}, ``Demonstration
  of {VR} / {AR} offloading to mobile edge cloud for low latency {5G} gaming
  application,'' in \emph{IEEE Annual Consumer Communications Networking
  Conference (CCNC)}, 2018, pp. 1--3.

\bibitem{Sultan18}
K.~Sultan, H.~Ali, and Z.~Zhang, ``Big data perspective and challenges in next
  generation networks,'' \emph{Future Internet}, vol.~10, no.~7, 2018.

\bibitem{Cisco19}
Cisco, ``Cisco visual networking index: Forcast and trends, 2017-2022,'' 2019.

\bibitem{you2016multiuser}
C.~You and K.~Huang, ``Multiuser resource allocation for mobile-edge
  computation offloading,'' in \emph{Proc. IEEE Global Communications
  Conference (GLOBECOM)}, 2016, pp. 1--6.

\bibitem{le2017efficient}
H.~Q. Le, H.~Al-Shatri, and A.~Klein, ``Efficient resource allocation in
  mobile-edge computation offloading: Completion time minimization,'' in
  \emph{IEEE International Symposium on Information Theory (ISIT)}, 2017, pp.
  2513--2517.

\bibitem{messaoudi2017using}
F.~Messaoudi, A.~Ksentini, and P.~Bertin, ``On using edge computing for
  computation offloading in mobile network,'' in \emph{Proc. IEEE Global
  Communications Conference (GLOBECOM)}, 2017, pp. 1--7.

\bibitem{li2019incentive}
L.~Li, T.~Q. Quek, J.~Ren, H.~H. Yang, Z.~Chen, and Y.~Zhang, ``An
  incentive-aware job offloading control framework for multi-access edge
  computing,'' \emph{IEEE Transactions on Mobile Computing}, 2019.

\bibitem{chen2018decentralized}
Z.~Chen and X.~Wang, ``Decentralized computation offloading for multi-user
  mobile edge computing: A deep reinforcement learning approach,'' \emph{arXiv
  preprint arXiv:1812.07394}, 2018.

\bibitem{cao2018joint}
X.~Cao, F.~Wang, J.~Xu, R.~Zhang, and S.~Cui, ``Joint computation and
  communication cooperation for energy-efficient mobile edge computing,''
  \emph{IEEE Internet of Things Journal}, 2018.

\bibitem{xing2019joint}
H.~Xing, L.~Liu, J.~Xu, and A.~Nallanathan, ``Joint task assignment and
  resource allocation for {D2D}-enabled mobile-edge computing,'' \emph{IEEE
  Transactions on Communications}, 2019.

\bibitem{molina2014joint}
M.~Molina, O.~Mu{\~n}oz, A.~Pascual-Iserte, and J.~Vidal, ``Joint scheduling of
  communication and computation resources in multiuser wireless application
  offloading,'' in \emph{IEEE International Symposium on Personal, Indoor, and
  Mobile Radio Communication (PIMRC)}, 2014, pp. 1093--1098.

\bibitem{wang2017computation}
C.~Wang, C.~Liang, F.~R. Yu, Q.~Chen, and L.~Tang, ``Computation offloading and
  resource allocation in wireless cellular networks with mobile edge
  computing,'' \emph{IEEE Transactions on Wireless Communications}, vol.~16,
  no.~8, pp. 4924--4938, 2017.

\bibitem{wang2017joint}
C.~Wang, F.~R. Yu, C.~Liang, Q.~Chen, and L.~Tang, ``Joint computation
  offloading and interference management in wireless cellular networks with
  mobile edge computing,'' \emph{IEEE Transactions on Vehicular Technology},
  vol.~66, no.~8, pp. 7432--7445, 2017.

\bibitem{wang2017joint2}
F.~Wang, J.~Xu, X.~Wang, and S.~Cui, ``Joint offloading and computing
  optimization in wireless powered mobile-edge computing systems,'' \emph{IEEE
  Transactions on Wireless Communications}, vol.~17, no.~3, pp. 1784--1797,
  2017.

\bibitem{barbarossa2017enabling}
S.~Barbarossa, E.~Ceci, M.~Merluzzi, and E.~Calvanese-Strinati, ``Enabling
  effective mobile edge computing using millimeterwave links,'' in \emph{IEEE
  International Conference on Communications Workshops (ICC Workshops)}, 2017,
  pp. 367--372.

\bibitem{sardellitti2015joint}
S.~Sardellitti, G.~Scutari, and S.~Barbarossa, ``Joint optimization of radio
  and computational resources for multicell mobile-edge computing,'' \emph{IEEE
  Transactions on Signal and Information Processing over Networks}, vol.~1,
  no.~2, pp. 89--103, 2015.

\bibitem{nguyen2019computation}
T.~T. Nguyen, L.~Le, and Q.~Le-Trung, ``Computation offloading in {MIMO} based
  mobile edge computing systems under perfect and imperfect {CSI} estimation,''
  \emph{IEEE Transactions on Services Computing}, 2019.

\bibitem{han2012subchannel}
M.-H. Han, B.-G. Kim, and J.-W. Lee, ``Subchannel and transmission mode
  scheduling for {D2D} communication in {OFDMA} networks,'' in \emph{IEEE
  Vehicular Technology Conference (VTC Fall)}, 2012.

\bibitem{wen2013energy}
S.~Wen, X.~Zhu, Z.~Lin, X.~Zhang, and D.~Yang, ``Energy efficient power
  allocation schemes for device-to-device ({D2D}) communication,'' in
  \emph{IEEE Vehicular Technology Conference (VTC Fall)}, 2013.

\bibitem{wang2013joint}
F.~Wang, L.~Song, Z.~Han, Q.~Zhao, and X.~Wang, ``Joint scheduling and resource
  allocation for device-to-device underlay communication,'' in \emph{IEEE
  wireless communications and networking conference (WCNC)}, 2013, pp.
  134--139.

\bibitem{zhao2017joint}
J.~Zhao, Y.~Liu, K.~K. Chai, Y.~Chen, and M.~Elkashlan, ``Joint subchannel and
  power allocation for {NOMA} enhanced {D2D} communications,'' \emph{IEEE
  Transactions on Communications}, vol.~65, no.~11, pp. 5081--5094, 2017.

\bibitem{6858049}
T.~{Kim} and M.~{Dong}, ``An iterative {Hungarian} method to joint relay
  selection and resource allocation for {D2D} communications,'' \emph{IEEE
  Wireless Communications Letters}, vol.~3, no.~6, pp. 625--628, 2014.

\bibitem{lin2015interplay}
X.~Lin, R.~W. Heath, and J.~G. Andrews, ``The interplay between massive {MIMO}
  and underlaid {D2D} networking,'' \emph{IEEE Transactions on Wireless
  Communications}, vol.~14, no.~6, pp. 3337--3351, 2015.

\bibitem{tang2013cooperative}
H.~Tang, C.~Zhu, and Z.~Ding, ``Cooperative {MIMO} precoding for {D2D} underlay
  in cellular networks,'' in \emph{IEEE International Conference on
  Communications (ICC)}, 2013, pp. 5517--5521.

\bibitem{wei2013device}
L.~Wei, R.~Q. Hu, T.~He, and Y.~Qian, ``Device-to-device ({D2D}) communications
  underlaying {MU}-{MIMO} cellular networks,'' in \emph{Proc. IEEE Global
  Communications Conference (GLOBECOM)}, 2013, pp. 4902--4907.

\bibitem{pu2016d2d}
L.~Pu, X.~Chen, J.~Xu, and X.~Fu, ``{D2D} fogging: An energy-efficient and
  incentive-aware task offloading framework via network-assisted {D2D}
  collaboration,'' \emph{IEEE Journal on Selected Areas in Communications},
  vol.~34, no.~12, pp. 3887--3901, 2016.

\bibitem{liu2018d2d}
J.~Liu, K.~Luo, Z.~Zhou, and X.~Chen, ``A {D2D} offloading approach to
  efficient mobile edge resource pooling,'' in \emph{IEEE International
  Symposium on Modeling and Optimization in Mobile, Ad Hoc, and Wireless
  Networks (WiOpt)}, 2018.

\bibitem{cover2012}
T.~M. Cover and J.~A. Thomas, \emph{Elements of information theory}.\hskip 1em
  plus 0.5em minus 0.4em\relax John Wiley \& Sons, 2012.

\bibitem{wen2012energy}
Y.~Wen, W.~Zhang, and H.~Luo, ``Energy-optimal mobile application execution:
  Taming resource-poor mobile devices with cloud clones,'' in \emph{IEEE
  International Conference on Computer Communications (INFOCOM)}, 2012, pp.
  2716--2720.

\bibitem{burer2012non}
S.~Burer and A.~N. Letchford, ``Non-convex mixed-integer nonlinear programming:
  A survey,'' \emph{Surveys in Operations Research and Management Science},
  vol.~17, no.~2, pp. 97--106, 2012.

\bibitem{chiang2007layering}
M.~Chiang, S.~H. Low, A.~R. Calderbank, and J.~C. Doyle, ``Layering as
  optimization decomposition: A mathematical theory of network architectures,''
  \emph{Proceedings of the IEEE}, vol.~95, no.~1, pp. 255--312, 2007.

\bibitem{scip2009}
T.~Achterberg, ``{SCIP}: Solving constraint integer programs,''
  \emph{Mathematical Programming Computation}, vol.~1, no.~1, pp. 1--41, 2009.

\bibitem{luo2008dynamic}
Z.-Q. Luo and S.~Zhang, ``Dynamic spectrum management: Complexity and
  duality,'' \emph{IEEE Journal of Selected Topics in Signal Processing},
  vol.~2, no.~1, pp. 57--73, 2008.

\bibitem{li2005distribution}
P.~Li, D.~Paul, R.~Narasimhan, and J.~Cioffi, ``On the distribution of {SINR}
  for the {MMSE MIMO} receiver and performance analysis,'' \emph{IEEE
  Transactions on Information Theory}, vol.~52, no.~1, pp. 271--286, 2005.

\bibitem{Qingjiangshi}
Q.~Shi, M.~Razaviyayn, Z.-Q. Luo, and C.~He, ``An iteratively weighted {MMSE}
  approach to distributed sum-utility maximization for a {MIMO} interfering
  broadcast channel,'' \emph{IEEE Transactions on Signal Processing}, vol.~59,
  no.~5, Sep 2011.

\bibitem{boyd2004convex}
S.~Boyd and L.~Vandenberghe, \emph{Convex optimization}.\hskip 1em plus 0.5em
  minus 0.4em\relax Cambridge university press, 2004.

\bibitem{au2007performance}
C.~K. Au-Yeung and D.~J. Love, ``On the performance of random vector
  quantization limited feedback beamforming in a {MISO} system,'' \emph{IEEE
  Transactions on Wireless Communications}, vol.~6, no.~2, pp. 458--462, 2007.

\bibitem{johnson2006modified}
S.~G. Johnson and M.~Frigo, ``A modified split-radix {FFT} with fewer
  arithmetic operations,'' \emph{IEEE Transactions on Signal Processing},
  vol.~55, no.~1, pp. 111--119, 2006.

\bibitem{ardito2013profiling}
L.~Ardito, G.~Procaccianti, M.~Torchiano, and G.~Migliore, ``Profiling power
  consumption on mobile devices,'' \emph{ENERGY}, pp. 101--106, 2013.

\bibitem{yetis2010}
C.~M. Yetis, T.~Gou, S.~A. Jafar, and A.~H. Kayran, ``On feasibility of
  interference alignment in {MIMO} interference networks,'' \emph{IEEE
  Transactions on Signal Processing}, vol.~58, no.~9, pp. 4771--4782, 2010.

\end{thebibliography}

==> related.tex <==
\section{Related Work}
\label{sec:related}
